FacePlex: Toward Natural Full-Duplex Conversational Avatars

Natural human conversation is inherently a real-time interaction in which speech and facial behavior continuously evolve. Enabling such interaction requires a conversational avatar to jointly generate speech and facial motion in real time, prepare facial motion for upcoming speech before the corresponding audio is emitted, and produce non-verbal reactions that reflect the ongoing dialogue. However, existing conversational avatar systems cannot address such requirements: audio-driven methods rely on pre-given speech, while joint streaming generation alone does not ensure anticipatory articulation or semantically appropriate reactions. We propose $\textbf{FacePlex}$, a unified framework for full-duplex speech-facial motion generation and real-time avatar rendering. FacePlex jointly coordinates speech, facial motion, and Gaussian splatting rendering on a shared streaming timeline. To prepare facial motion for upcoming speech, FacePlex predicts a short speech continuation and uses its future hidden states through asymmetric conditioning and denoising, while continuously updating them as new user audio arrives without observing future user input. For dialogue-grounded non-verbal behavior, we construct $\textit{SemReact}$, a dataset aligning dialogue context, reaction semantics, and facial motion, and introduce a semantic behavior router that guides continuous motion during both speaking and listening. Extensive experiments show improved audio-visual synchronization and facial articulation, natural dialogue-grounded non-verbal responses, and low-latency of 122 ms end-to-end avatar interaction.

==> Sections/8_Method_Details.tex <==
\section{Streaming Generation Details}
\label{app:streaming_details}

\subsection{Motion Network}
\label{app:motion_architecture}

The shared velocity network $\VelocityField$, parameterized by trainable weights $\MotionParams$, has eight transformer layers, width $\MotionWidth=512$, and eight attention heads.
The generator maintains $\ActiveFrameCount=8$ noisy motion frames, grouped into $\QueueLength=4$ pairs.
Each pair contains two tokens and corresponds to one 80\,ms streaming step.
Persona tokens $\PersonaTokens$ and style tokens $\StyleTokens{\StreamIndex}$ each represent a 100-frame reference motion clip, one token per frame.
The persona reference and its tokens remain fixed throughout a session.
The bank lookup $\StyleRouter$ selects the style reference matching the reaction class and own-speech flag.
History tokens represent the eight previous completed frames, while eight motion tokens represent the current noisy frames.
All four token types use the same framewise linear projection $\MotionProjection$ from $\MotionDim=108$ coordinates to width $\MotionWidth=512$, implemented by a single shared \texttt{nn.Linear(108, 512)} layer.
Token-type embeddings distinguish motion, history, and reference inputs; additional reference-type embeddings distinguish persona tokens from style tokens.
These are continuous feature vectors, each representing one 108-dimensional FLAME frame.
Each motion token $\MotionToken{\MotionFrameIndex}$ combines projected noisy coordinates with token-type and group-specific flow-time embeddings.
Embeddings of behavior, the own-speech flag, and gesture phase provide the controls described in Sec.~\ref{sec:semantic_behavior}.

Within each layer, motion self-attention combines motion tokens with history, persona, and style tokens.
Joint self-attention operates on the motion tokens and the four hidden states projected by $\SpeechProjection\in\R^{\MotionWidth\times\SpeechDim}$.
We denote the history tokens, persona tokens, style tokens, and framewise controls collectively by $\MotionConditions$, with the hidden-state window supplied separately.
Only the motion outputs are retained as residual updates, followed by a feed-forward block.
The longer conversational memory is used by the router; its states are not added to this short speech window.

\subsection{Run-Ahead Buffer and Cache}
\label{app:run_ahead_details}

Figure~\ref{fig:run_ahead_buffer_cache} illustrates how sequential warm-up prepares the token buffer and how batched run-ahead $\BatchedRunAhead$ updates the hidden states after each user observation.
During warm-up, each backbone hidden state is passed to the depth transformer, and the resulting user and avatar tokens become inputs for the next step.
This sequential rollout continues until the buffer contains the required input window.
The buffer stores avatar audio and text tokens, temporary user audio tokens, and incomplete entries for delayed codebooks.
At each step, the current user prediction is replaced by the observed tokens as described in Sec.~\ref{sec:run_ahead}, while the avatar audio and text tokens remain fixed.
If codebook entries required for the next window are incomplete, they are filled sequentially before batched evaluation.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Method1.pdf}
    \caption{Run-ahead prediction and hidden-state updates.
    \textbf{(a)} Sequential warm-up feeds predicted user tokens $\PredictedUserAudioTokens{i}$ and generated avatar audio tokens $\AvatarTokens{i}$ back into the backbone to prepare a short continuation.
    \textbf{(b)} As observed user tokens $\UserAudioTokens{i}$ arrive, they replace their predictions while avatar tokens remain fixed.
    The temporal transformer recomputes the buffered window in one causal pass, and only the last hidden state invokes the depth transformer (depformer) to extend the buffer.
    Primes mark hidden states recomputed after new user observations.
    Cyan tokens are user predictions; red-bordered tokens are observed user inputs or committed avatar outputs.
    Completed history is reused through the KV cache, while the window's cache entries are refreshed.}
    \label{fig:run_ahead_buffer_cache}
\end{figure}

Once the buffer is filled, the temporal transformer can read all rows in the window together: their token values are already known, and causal attention preserves their temporal order.
At processing step $\StreamIndex$, a single causal transformer pass reads input rows $\StreamIndex,\ldots,\StreamIndex+\RunAheadHorizon$ from $\UpdatedTokenBuffer_{\StreamIndex}$ using $\SpeechCache$ and produces states at positions $\StreamIndex+1,\ldots,\StreamIndex+\RunAheadHorizon+1$.
Only the last state $\ProvisionalHidden_{\StreamIndex+\RunAheadHorizon+1\mid\StreamIndex}$ is passed to the output heads and depth transformer to generate $\PredictedUserAudioTokens{\StreamIndex+\RunAheadHorizon+1}$ and $\AvatarTokens{\StreamIndex+\RunAheadHorizon+1}$, as returned by $\BatchedRunAhead$ in Sec.~\ref{sec:run_ahead}.
Here $\AvatarTokens{\StreamIndex+\RunAheadHorizon+1}$ denotes avatar audio tokens; the accompanying text tokens are also generated but omitted from the notation.
Appending the generated audio and text tokens extends the buffer to position $\StreamIndex+\RunAheadHorizon+1$.
For the same tokens, cache, positions, and attention mask, this computation matches sequential evaluation up to numerical precision.
This equivalence concerns evaluation of the same buffered inputs; it does not imply equivalence to decoding with actual future user audio.
The sequential warm-up takes about 85\,ms in our implementation, and a subsequent batched pass takes about 25\,ms.
% TODO: identify hardware, measured operations, and repetition counts for these timings.

The KV cache stores each layer's keys and values for earlier input rows, allowing later rows to attend to that history without recomputing it.
Entries preceding $\StreamIndex$ depend on already observed user audio and committed avatar tokens, so they can be reused.
After replacing $\PredictedUserAudioTokens{\StreamIndex}$ with $\UserAudioTokens{\StreamIndex}$, the transformer recomputes the keys and values at input position $\StreamIndex$.
Through causal attention, this update can affect hidden states and keys and values at all later positions in the window, so the window is recomputed while $\SpeechCache$ is reused.
Cache entries correspond to input positions, whereas hidden-state indices denote next-token positions.
After extracting the hidden-state window, we retain the recomputed keys and values for input position $\StreamIndex$ in $\SpeechCache$, extending the observed history for the next pass.
At step $\StreamIndex+1$, the newly observed user token produces $\DialogueHidden{\StreamIndex+2}$ and refreshes the overlapping future states:
\begin{equation}
    \begin{aligned}
        \ProvisionalHidden_{\StreamIndex+2\mid\StreamIndex}&\rightarrow\DialogueHidden{\StreamIndex+2}, \\
        \ProvisionalHidden_{\StreamIndex+\FutureOffset\mid\StreamIndex}
        &\rightarrow\ProvisionalHidden_{\StreamIndex+\FutureOffset\mid\StreamIndex+1},
        \quad \FutureOffset=3,\ldots,\RunAheadHorizon+1.
    \end{aligned}
    \label{eq:run_ahead_update}
\end{equation}
The new window also adds $\ProvisionalHidden_{\StreamIndex+\RunAheadHorizon+2\mid\StreamIndex+1}$ at its far end.
Only the cache entry for the newly observed input row is retained as completed history; future entries remain provisional and are overwritten on the next pass.
Because the cache is a ring buffer, a future-position write can land on a slot that still holds valid history.
We snapshot such slots before the pass and restore them afterwards.
The token buffer and motion queue persist across steps.

\subsection{Consistency Between Committed Speech and Updated States}
\label{app:run_ahead_consistency}

During run-ahead prediction, we use the same committed avatar tokens to produce the speech played to the user and to recompute the hidden states that condition motion.
We distinguish the effect of committing speech early from the effect of updating its motion-conditioning states.
The speech comparisons branch from the same ground-truth dialogue history and allow avatar predictions to differ: they measure how waiting for actual future user audio would change the speech continuation.
Their token-disagreement rates do not measure mismatches between played audio and motion conditioning.

\para{Greedy speech agreement.}
% Source supplied by the author: outputs/analysis/lockin_summary.md.
We evaluate 50 Seamless Interaction validation windows containing 7,550 frames.
From the same ground-truth history, branch S predicts the next user frames with the speech backbone, while branch R receives the actual user frames.
Both branches generate avatar tokens using greedy decoding.
Branch R is a counterfactual used for this evaluation; its avatar predictions do not replace committed tokens in the run-ahead system.
Table~\ref{tab:run_ahead_token_agreement} reports agreement between these branches at three future positions.
At 240\,ms, 4.3\% of semantic tokens differ, compared with 2.1\% of text tokens and 21.0\% of acoustic tokens.
Semantic-token agreement with the ground-truth conversation is nearly unchanged: 0.436 for S and 0.435 for R.
The perfect semantic agreement at 80\,ms follows from the decoder ordering, in which avatar codebooks precede user codebooks in the depth transformer.
These are greedy prediction comparisons; we did not measure token-change rates under sampling.

\begin{table}[t]
    \centering
    \small
    \caption{Counterfactual comparison of greedy avatar predictions under predicted (S) and observed (R) user input. The first three agreement columns compare these speech continuations; the last two compare semantic predictions with ground-truth tokens.}
    \label{tab:run_ahead_token_agreement}
    \begin{tabular}{rccccc}
        \toprule
        & \multicolumn{3}{c}{S--R agreement} & \multicolumn{2}{c}{Semantic agreement with GT} \\
        \cmidrule(lr){2-4}\cmidrule(lr){5-6}
        Ahead (ms) & Text & Semantic & Acoustic & R & S \\
        \midrule
        +80  & 1.000 & 1.000 & 0.920 & 0.573 & 0.573 \\
        +160 & 0.993 & 0.983 & 0.839 & 0.486 & 0.487 \\
        +240 & 0.979 & 0.957 & 0.790 & 0.435 & 0.436 \\
        \bottomrule
    \end{tabular}
\end{table}

\para{Speech distribution overlap.}
% Source supplied by the author: outputs/analysis/paper_csv/runahead_dist_overlap.csv.
To compare the full next-token distributions, we sample 2,080 probes from 80 clips at six-frame intervals, again starting from the same ground-truth history for each comparison.
We compare predicted user input (S), repetition of the last observed user frame (H), and an unrelated user frame (W), each against actual user input (R).
For distributions $p$ and $q$, we report overlap $\sum_v\min\{p(v),q(v)\}$, equal to one minus total variation, and Jensen--Shannon (JS) divergence in bits.
Table~\ref{tab:run_ahead_distribution} also reports semantic top-1 agreement.

At 240\,ms, S retains 0.979 text overlap and 0.970 semantic overlap, with JS divergences of 0.0034 and 0.0058 bits, respectively.
For speaking frames alone, text and semantic overlap are 0.988 and 0.980 at 160\,ms, and 0.977 and 0.962 at 240\,ms.
Top-1 agreement here is measured on these 2,080 probes, separately from the greedy rollout evaluation above.
Even W retains more than 0.93 overlap at 240\,ms, suggesting that the existing dialogue history strongly constrains the immediate speech predictions.
Together, these results support short-term stability of text and semantic predictions across these input conditions, while acoustic tokens differ more between the counterfactual speech continuations.
Already committed avatar tokens cannot be revised in response to later user input.

\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{5pt}
    \caption{Avatar next-token distributions relative to observed user input (R). S uses predicted user frames, H repeats the last observed frame, and W uses an unrelated frame. Overlap and semantic top-1 agreement are fractions; JS divergence is in bits.}
    \label{tab:run_ahead_distribution}
    \begin{tabular}{lrccccc}
        \toprule
        & & \multicolumn{2}{c}{Text} & \multicolumn{3}{c}{Semantic} \\
        \cmidrule(lr){3-4}\cmidrule(lr){5-7}
        User input & Ahead (ms) & Overlap & JS & Overlap & JS & Top-1 \\
        \midrule
        S: predicted & +160 & 0.990 & 0.0013 & 0.983 & 0.0026 & 0.980 \\
        S: predicted & +240 & 0.979 & 0.0034 & 0.970 & 0.0058 & 0.964 \\
        H: last observed & +240 & 0.979 & 0.0032 & 0.970 & 0.0053 & 0.960 \\
        W: unrelated & +240 & 0.931 & 0.0210 & 0.934 & 0.0162 & 0.933 \\
        \bottomrule
    \end{tabular}
\end{table}

\subsection{Numerical Motion Updates}
\label{app:motion_updates}

We split each frame into expression--jaw ($\ExpressionJawGroup$, 101 coordinates) and head--eye ($\HeadEyeGroup$, seven coordinates).
The expression--jaw group includes all expression coefficients, including the upper face.
Each group has its own flow time, from noise at $\FlowTime=0$ to clean motion at $\FlowTime=1$.
At processing step $\StreamIndex$, we output the pair for position $\StreamIndex$, completed at step $\StreamIndex-1$, and use its frames to update the history tokens.
We shift the queue forward and insert a new noise pair at the rear, so the active pairs target output positions $\StreamIndex+1,\ldots,\StreamIndex+\QueueLength$.
Head--eye flow times start at $[3/4,1/2,1/4,0]$ from front to rear.
The two shared updates each advance these times by $1/8$.
Expression--jaw coordinates remain at the noise source in the rear three pairs and complete their refinement in the front pair.

The queue contains $\QueueLength=4$ pairs, and each streaming step uses $\SharedSteps=2$ shared network evaluations.
These evaluations update head--eye coordinates in all pairs and expression--jaw coordinates in the front pair.
When $\DialogueState{\StreamIndex}=1$, another $\ExtraSteps=2$ evaluations update only the front pair's expression--jaw coordinates.
The expression--jaw update count is therefore
\begin{equation}
    \ExpressionJawSteps(\StreamIndex)=\SharedSteps+\ExtraSteps\DialogueState{\StreamIndex}=2+2\DialogueState{\StreamIndex},
    \label{eq:state_refinement_budget}
\end{equation}
giving four updates during avatar speech and two otherwise, including mutual silence.
The schedule in Eq.~\ref{eq:asymmetric_update_counts} shows the speaking case.
Head--eye coordinates and flow times remain fixed during the extra evaluations.
At inference, $\DialogueState{\StreamIndex}$ is the router's speaking/listening decision made at processing step $\StreamIndex$ for the output at $\StreamIndex+1$; during training, speaking-state conditioning comes from the framewise labels of the data.
Applying the extra updates in all states improved speaking expression dynamics but worsened listening dynamics, so the extra updates are gated by the own-speech flag.

Let $\NoisyMotion$ be the full noisy queue, $\FlowTimes$ its group flow times, $\SpeechWindow$ the hidden-state window, and $\GroupStepSize$ the step size for group $\MotionGroupIndex$.
During streaming, $\SpeechWindow=\OnlineSpeechWindow_{\StreamIndex}$.
We apply Euler updates to the selected coordinates:
\begin{equation}
    \NoisyMotion_{\MotionFrameIndex}^{\MotionGroupIndex}\leftarrow
    \NoisyMotion_{\MotionFrameIndex}^{\MotionGroupIndex}
    +\GroupStepSize\left[\FrameVelocity{\MotionFrameIndex}
    (\NoisyMotion;\FlowTimes,\SpeechWindow,\MotionConditions)\right]^{\MotionGroupIndex}.
    \label{eq:group_refinement}
\end{equation}
The head--eye step size is $\HeadEyeStepSize=1/(\QueueLength\SharedSteps)=1/8$.
For expression--jaw motion, it is $\ExpressionJawStepSize(\StreamIndex)=1/\ExpressionJawSteps(\StreamIndex)$.
Both schedules finish at flow time one.
All evaluations call the full shared network.
Shared evaluations use $\SharedConditions$, which includes history, persona, and style tokens, the current state, reaction, and phase labels, and the labels carried by history tokens.
Extra evaluations use $\ExtraConditions$: the three context token types remain, but the current state, reaction, and phase labels are zero and the history label embeddings are omitted.
Both evaluations use the same hidden-state window.
The evaluated policy includes this conditioning difference, so the effect of the extra updates is not attributed to integration step size alone.

\subsection{Motion Training}
\label{app:motion_training}

For clean motion $\CleanMotion_{\MotionFrameIndex}$ and Gaussian noise $\MotionNoise_{\MotionFrameIndex}\sim\mathcal{N}(0,\IdentityMatrix_{\MotionDim})$, the training path is
\begin{equation}
    \NoisyMotion_{\MotionFrameIndex}^{\MotionGroupIndex}
    =(1-\FlowTime_{\MotionFrameIndex}^{\MotionGroupIndex})\MotionNoise_{\MotionFrameIndex}^{\MotionGroupIndex}
    +\FlowTime_{\MotionFrameIndex}^{\MotionGroupIndex}\CleanMotion_{\MotionFrameIndex}^{\MotionGroupIndex},
    \qquad \MotionGroupIndex\in\{\ExpressionJawGroup,\HeadEyeGroup\}.
    \label{eq:asymmetric_flow_path}
\end{equation}
The superscript $\MotionGroupIndex$ selects a group's coordinates.
Together, the groups form a noisy frame $\NoisyMotion_{\MotionFrameIndex}\in\R^{\MotionDim}$.
We train the network to predict the displacement from noise to clean motion:
\begin{equation}
    \MotionFlowLoss=
    \E\!\left[
    \frac{1}{\ActiveFrameCount\MotionDim}\sum_{\MotionFrameIndex=1}^{\ActiveFrameCount}
    \left\|\FrameVelocity{\MotionFrameIndex}(\NoisyMotion;\FlowTimes,\SpeechWindow,\MotionConditions)
    -(\CleanMotion_{\MotionFrameIndex}-\MotionNoise_{\MotionFrameIndex})\right\|_2^2\right].
    \label{eq:rolling_fm_loss}
\end{equation}
Here $\NoisyMotion$ is the noisy queue and $\FlowTimes$ collects its group flow times.
The loss averages velocity errors over all eight frames and 108 coordinates.

We sample noisy inputs directly from Eq.~\ref{eq:asymmetric_flow_path}, without unrolling the inference updates.
For head--eye motion, the four pairs start at flow times $[3/4,1/2,1/4,0]$.
We add the same random offset, uniform over $[0,1/4]$, to these times.
For expression--jaw motion, we independently sample the front pair's time uniformly over $[0,1]$ and keep the rear pairs at zero.
Both frames in a pair share their group flow times.
All coordinates receive velocity supervision, including expression--jaw coordinates at flow time zero in the rear pairs.

Each training crop contains eight history frames and two consecutive eight-frame target chunks.
We evaluate the chunks separately, using their preceding ground-truth frames to form history tokens, and average their losses.
The second chunk does not use generated motion from the first.
The state-dependent update count is used only during inference.

We initialize from a listener model with the same persona and style token inputs.
We train the motion generator and router, keeping the speech backbone and codec frozen.
Training combines synthetic speaking motion, real conversations from Seamless Interaction, and labeled synthetic reaction motion.
Section~\ref{sec:semantic_behavior} adds the reaction-routing objective.
% TODO (Appendix): Specify the initialization checkpoint, optimizer, learning-rate
% schedule, dataset sampling ratios, batch size, training steps, and random seeds.

\subsection{Hidden-State Timing Probe}
\label{app:hidden_state_probe}

For the analysis in Fig.~\ref{fig:future_context_analysis}(a), we extract hidden states from the frozen speech backbone on Seamless Interaction~\citep{agrawal2025seamless} conversations.
We fit ridge regression models to predict motion at a target pair's position, each using a single hidden state at a specified temporal offset.
We compare past, current, and future positions relative to the target, with one step corresponding to 80\,ms.
The regressions are fitted on training data and evaluated on a separate test set.
We report the coefficient of determination $\ProbeRSquared$ for jaw, expression, head, and eye motion; higher values indicate more accurate predictions from the selected hidden state.
These scores characterize the predictive information available to a linear model at each offset.
% TODO (Probe reproducibility): Confirm the final Figure 3(a) data count and
% train/validation/test split, feature and target normalization, ridge penalty
% selection, two-frame target aggregation, and multi-coordinate R^2 aggregation
% against the analysis code. Sections/Supples/1.tex is an older, uncompiled note.


==> Sections/Supples/1.tex <==
# Paper text — future-context analysis (Figure: hidden-time correlation / window extension / trained controls)

## Figure caption (main text)

**Figure X. Speaking motion depends on the next 80–240 ms of the speech model's hidden state; listening motion does not.**
All panels share the same time axis: the offset of a hidden state h_{T+k} relative to the motion frame T (k·80 ms; positive = future).
The shaded band marks the conditioning window used by our model, [h_T, …, h_{T+3}].
**(a)** Held-out R² of a ridge probe that predicts the ground-truth motion at frame T from a *single* hidden state h_{T+k}, on Seamless Interaction (1,100 clips, 16 s each; see Supp. §S1). Speaking-frame jaw (and expression) is explained best by h_{T+1}…h_{T+3}; listening-frame head pose is not explained by any offset.
**(b)** The same probe with a *window* of hidden states, extended from h_T either into the future ([h_T … h_{T+x}]) or into the past ([h_{T−x} … h_T]). Future slots add explained variance (0.22 → 0.40 with one slot, saturating at three = our window); past slots add none.
**(c)** Lip-sync of flow-matching motion models trained with the same recipe but with the 4-slot window shifted from the past to the future (S-LVE, lower is better; PLRS, higher is better; seamless, n = 500). The dotted line is our model evaluated with its future slots left empty at inference. Quality follows the data-side curves and saturates at a lookahead of 240 ms.
Because the speech model emits h_{T+1} only after reading the audio codes of frame T (acoustic codebooks are delayed by one more step), a window ending at h_T contains no information about the sound being produced at T.

## Supplementary §S1 — Data-side analysis of future dependence

**Data.** We use the validation split of Seamless Interaction that was never used to train the motion model: 550 dyadic sessions, both participants, i.e. 1,100 clips of 16 s. For every clip we have (i) ground-truth FLAME motion at 25 fps (108-D: 100 expression, 3 head rotation, 1 jaw, 4 gaze), (ii) the participant's own and the partner's 16 kHz audio, and (iii) the hidden states of the full-duplex speech LM (PersonaPlex-7B, Moshi architecture) obtained by teacher-forcing the real conversation through the model: the participant's speech on the model's own stream and the partner's speech on the user stream. Hidden states are the 4096-D temporal-transformer outputs at 12.5 Hz (one per 80 ms frame), exactly the conditioning our motion model receives at inference. Motion is averaged over the two 25-fps frames of each 80 ms step so that motion and hidden states share one clock.

**Timing convention.** The transformer at step s reads the token row at position s − 1, and the acoustic codebooks are delayed by one frame relative to the semantic codebook. Hence h_T has read the participant's semantic codes up to frame T − 1 and acoustic codes up to T − 2; h_{T+1} is the first state that contains the sound of frame T, and h_{T+2} the first that contains its acoustic detail. All offsets are reported in hidden-state time; in audio time the peak of (a) lies 80–160 ms earlier.

**Frame classes.** A frame is *speaking* if the participant's own audio RMS exceeds 0.003 (the threshold used by the benchmark), and *listening* if the participant is silent and the partner's RMS exceeds 0.003. Frames satisfying neither are excluded.

**Probe.** For each offset k ∈ {−6, …, +6} we fit a ridge regression from h_{T+k} (standardized per dimension) to the motion at frame T. Targets are standardized per clip (each clip's mean and standard deviation removed) so that the probe measures timing information rather than a participant's average pose. Clips are split 70 / 10 / 20 % into train / validation / test; the ridge coefficient is fit on the train clips, the regularization strength is chosen on the validation clips from {10¹, …, 10⁵}, and we report R² = 1 − SSE/SST on the **held-out** test clips. R² is computed jointly over the dimensions of a target group (jaw; expression 0–99; head 100–102; gaze 103–106). For panel (b) the hidden state of each slot is first reduced to 512 dimensions by PCA fitted on training clips, and the slots of a window are concatenated before ridge regression; alpha selection and held-out evaluation are as above. Held-out R² is a lower bound on the information the hidden states carry, since the probe is linear and sees no context beyond the window.

**Trained controls (panel c).** Nine motion models were trained with one recipe (initialized from the adopted asymmetric-schedule checkpoint, 100k steps, learning rate 5·10⁻⁵, single-chunk windows, evaluated with K = 4 refinement passes) that differ only in the position of their 4-slot conditioning window: [h_{T−3−j} … h_{T−j}] for j = 6, 3, 2, 1 (windows entirely in the past), the causal window [h_{T−3} … h_T], and [h_{T−2} … h_{T+1}], [h_{T−1} … h_{T+2}], [h_T … h_{T+3}] (ours); two further models extend the window to five and six slots ([h_T … h_{T+4}], [h_T … h_{T+5}]). All are evaluated on the same 500 seamless windows (seed 20260426, full audio rollout capped at 288 motion frames, paired). Training-seed noise for this recipe is ≈ 0.35 mm S-LVE and ≈ 0.002 PLRS (three seeds of the [h_T … h_{T+3}] model: 7.09 / 6.74 / 6.94 mm), so S-LVE differences among windows reaching ≥ 160 ms are within noise and only PLRS separates them. The dotted reference (S-LVE 9.40, PLRS 0.171) is the adopted model with its three future slots left empty at inference.

**Additional observations (not in the figure).** With raw 40-band log-mel of the participant's own audio as the input instead of hidden states, the speaking-jaw probe peaks sharply at 0–80 ms (r = 0.37) and falls below r = 0.13 outside ±160 ms, confirming the 80–160 ms shift between audio time and hidden-state time. Listening-frame jaw shows a weak, broad dependence (r ≈ 0.2, slightly higher for future states) that we attribute to silent mouth preparation before the next turn; listening head pose and gaze show none (R² ≤ 0) for single states, for 1-s windows of partner speech, and for windows extended in either direction. Data files: `outputs/analysis/paper_csv/fig_{a,b,c}_*.csv`, `window_ablation_all.csv`; scripts: `scripts/analysis/{audio_time_correlation*.py, future_context_hidden_time.py, audio_window_dose_response.py}`.


==> Tables/ablation_horizon_attention.tex <==
% Horizon table; attention/SemReact variants are now in the component table.
\begin{table}[!htbp]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{2pt}
    \caption{Hidden-state horizon $\RunAheadHorizon$.}
    \label{tab:ablation_horizon}
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{1}
    \setlength{\aboverulesep}{1.5pt}
    \setlength{\belowrulesep}{1.5pt}
    \input{Tables/tab_ablation_horizon}
    \par\vspace{2pt}
    All metrics $\downarrow$; time: online compute in ms/step (separate probe); gray: FacePlex configuration.
\end{table}


==> Tables/ablation_horizon_routing.tex <==
% Horizon and semantic-routing tables share a row, with separate captions.
\begin{table}[!htbp]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{2pt}
    \begin{minipage}[t]{0.49\linewidth}
        \vspace{0pt}
        \caption{Hidden-state horizon $\RunAheadHorizon$.}
        \label{tab:ablation_horizon}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.49\linewidth}
        \vspace{0pt}
        \caption{Semantic routing; speaking/listening decisions fixed.}
        \label{tab:ablation_semantic_routing}
    \end{minipage}
    \par
    \fontsize{7}{8}\selectfont
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{1}
    \setlength{\aboverulesep}{1.5pt}
    \setlength{\belowrulesep}{1.5pt}
    \begin{minipage}[t]{0.49\linewidth}
        \vspace{0pt}
        \input{Tables/tab_ablation_horizon}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.49\linewidth}
        \vspace{0pt}
        \input{Tables/tab_ablation_semantic_routing}
    \end{minipage}
    \par\vspace{2pt}
    All metrics $\downarrow$. Left: time is online compute in ms/step (separate probe); gray marks the FacePlex configuration.
    Right: samples from the Seamless Interaction test split; fixed checkpoint; gray marks the paired default. Ours is the separate Table~\ref{tab:main} reference.
\end{table}


==> Tables/ablation_latency_window.tex <==
% Compact latency and window-placement tables retain separate table numbers.
\begin{table}[H]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{2pt}
    \begin{minipage}[t]{0.34\linewidth}
        \vspace{0pt}
        \caption{Mean server-side audio/motion availability delay.}
        \label{tab:ablation_run_ahead_latency}
    \end{minipage}\hfill
    \begin{minipage}[t]{0.64\linewidth}
        \vspace{0pt}
        \caption{Placement of a window of four hidden states; offsets in 80\,ms steps.}
        \label{tab:ablation_window_position}
    \end{minipage}
    \par
    \fontsize{7}{8}\selectfont
    \setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{1}
    \setlength{\aboverulesep}{1.5pt}
    \setlength{\belowrulesep}{1.5pt}
    \begin{minipage}[t]{0.34\linewidth}
        \vspace{0pt}
        \input{Tables/tab_ablation_run_ahead_latency}
        \par\vspace{2pt}
        Includes capture and queueing; excludes rendering. Main-table input-plus-forward latency: 0.122\,s.
    \end{minipage}\hfill
    \begin{minipage}[t]{0.64\linewidth}
        \vspace{0pt}
        \input{Tables/tab_ablation_window_position}
        \par\vspace{2pt}
        All metrics $\downarrow$.
    \end{minipage}
\end{table}


==> Tables/ablation_semantic_routing.tex <==
% Compact semantic-routing table; SemReact training is included in Table 6.
\begin{table}[!htbp]
    \centering
    \fontsize{8}{9}\selectfont
    \setlength{\abovecaptionskip}{0pt}
    \setlength{\belowcaptionskip}{2pt}
    \begin{minipage}{0.54\linewidth}
        \centering
        \caption{Semantic routing; speaking/listening decisions fixed.}
        \label{tab:ablation_semantic_routing}
        \fontsize{7}{8}\selectfont
        \setlength{\tabcolsep}{1pt}
        \renewcommand{\arraystretch}{1}
        \setlength{\aboverulesep}{1.5pt}
        \setlength{\belowrulesep}{1.5pt}
        \input{Tables/tab_ablation_semantic_routing}
        \par\vspace{2pt}
        Samples from the Seamless Interaction test split; fixed checkpoint; all metrics $\downarrow$.
        Gray: paired default. Ours: the separate Table~\ref{tab:main} reference.
    \end{minipage}
\end{table}


==> Tables/fig_app_example.tex <==
\begin{figure}[p]
    \centering
    \includegraphics[
        width=0.95\linewidth,
        height=0.42\textheight,
        keepaspectratio
    ]{Figures/Experiments/appendix_session_example1.pdf}

    \includegraphics[
        width=0.95\linewidth,
        height=0.42\textheight,
        keepaspectratio
    ]{Figures/Experiments/appendix_session_example2.pdf}

    \caption{
    More qualitative results of \textbf{FacePlex}.
    We visualize additional generated facial-motion sequences with the corresponding phonetic and prosodic cues shown above each sequence.
    Best viewed with zoom.
    }
    \label{fig:app_more_qualitative}
\end{figure}


==> Tables/tab_ablation_attention.tex <==
% Archived body of the former Table 6; not included in the compiled paper.
% Active rows are merged into Tables/tab_ablation_recomputation_schedule.tex.
% Source: https://app.notion.com/p/3e5036874646818f8027dd0cbff63187
% Cross-attention retains the V9 fusion scratch100K evaluation, original_intervals_self_v2.
% Joint self-attention now uses final FacePlex means from Tables/main.tex at
% the author's request (2026-09-26); the two rows no longer form a matched100K pair.
% Full precision (S-LVE, S-MHD, S-FDD, L-FDD, L-FID):
% Cross: 7.41788, 1.72124, 24.02670, 28.72838, 1.73348.
% Previous joint scratch100K: 7.46424, 1.74890, 24.89938, 30.25608, 1.67140.
% Current joint: 7.162, 1.674, 22.839, 26.623, 1.407 (main-table displayed means).
% SemReact training comparison (formerly Table 10):
% w/o SemReact: author-supplied 2026-09-26 values 7.57, 1.73, 24.3, 25.1, 0.759.
% w/ SemReact: the same final FacePlex means from Tables/main.tex.
% Matched training/evaluation settings for these comparisons remain to be verified.
\begin{tabularx}{\linewidth}{@{}l*{5}{>{\centering\arraybackslash}X}@{}}
    \toprule
    Setting & S-LVE & S-MHD & S-FDD & L-FDD & L-FID \\
    \midrule
    Cross-attn. & 7.418 & 1.721 & 24.027 & 28.728 & 1.733 \\
    \rowcolor{lightgray!40}
    Joint self-attn. (Ours) & 7.162 & 1.674 & 22.839 & 26.623 & 1.407 \\
    \midrule
    w/o SemReact & 7.570 & 1.730 & 24.300 & 25.100 & 0.759 \\
    \rowcolor{lightgray!40}
    w/ SemReact & 7.162 & 1.674 & 22.839 & 26.623 & 1.407 \\
    \bottomrule
\end{tabularx}


==> Tables/tab_app_latency_components.tex <==
% Source: outputs/h200_fm_compile_20260926/audit.json; speaking means only.
\begin{table}[!htbp]
    \centering
    \begin{minipage}{0.70\linewidth}
        \centering
        \small
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{3pt}
        \caption{Optimized H200 mean processing time while speaking (ms). Total combines input acquisition and forward computation, excluding rendering. Forward is measured separately and includes stream bookkeeping and CPU audio/FLAME availability. Total adds the configured 80\,ms input interval. Both exclude mesh construction, rendering, network, and client playback.}
        \label{tab:latency_components}
        \fontsize{8}{9}\selectfont
        \setlength{\tabcolsep}{3pt}
        \renewcommand{\arraystretch}{1}
        \begin{tabularx}{\linewidth}{@{}Xr@{}}
            \toprule
            Component & Time (ms) \\
            \midrule
            Input buffering (configured) & 80.00 \\
            Mimi encode & 3.20 \\
            Temporal transformer & 11.90 \\
            Depth transformer & 11.86 \\
            Semantic and style routing & 0.23 \\
            Motion generator & 7.43 \\
            Mimi decode & 2.32 \\
            \midrule
            Forward (separate pass) & 42.16 \\
            Total (Input + Forward) & 122.16 \\
            \bottomrule
        \end{tabularx}
    \end{minipage}
\end{table}


==> Tables/tab_app_runahead_timing.tex <==
% CPU verification of the completed speaking4/listening2 traces (396 runs total):
% outputs/paper_ablation_20260926/timing_state_gated42/verified_results.json.
% Rows: k3_full_wait_reference, k3_sequential_matched, k3_batched_matched.
% FM is eager. Full-wait is a separate task/hardware allocation; only the
% sequential/batched pair shares the same physical GPU and stage instrumentation.
\begin{table}[!htbp]
    \centering
    \small
    \caption{Run-ahead timing with one H200 per run, 22 input sessions, and two seeds (5,318 scored pairs per condition). Full-wait is a separate reference profile; the replay rows form the matched comparison. Compute is synchronized streaming-step wall time; AV delay is measured from the corresponding input interval to CPU audio and FLAME availability. Startup is included; rendering, network, and playback are excluded.}
    \label{tab:app_runahead_timing}
    \begin{tabular}{lrr}
        \toprule
        Condition & Compute (ms/step) & Mean AV delay (ms) \\
        \midrule
        Full-wait & \textbf{48.94} & 369.84 \\
        Sequential self-replay & 116.67 & 2488.02 \\
        Batched run-ahead & 55.74 & \textbf{140.78} \\
        \bottomrule
    \end{tabular}
\end{table}


==> Tables/tab_app_schedule_variation.tex <==
% Source: outputs/paper_ablation_20260926/gated42/diagnostics/progressive_motion_comparison.json.
% All 479 eligible speaking clips, equal clip weights; no smoothing/rescaling.
\begin{table}[!htbp]
    \centering
    \caption{Mean temporal standard deviation over speaking frames in evaluated clips from the Seamless Interaction test split. Expression variation is averaged over its 100 coefficients. These are raw FLAME coefficient statistics.}
    \label{tab:app_schedule_variation}
    \begin{tabular}{lrr}
        \toprule
        Condition & Jaw & Expression \\
        \midrule
        Progressive, updates off & 0.03148 & 0.11561 \\
        Progressive, updates on & 0.03150 & 0.11572 \\
        Late, state-gated (paired default) & 0.04184 & 0.16574 \\
        Recorded reference & 0.04518 & 0.20324 \\
        \bottomrule
    \end{tabular}
\end{table}

